The buoyancy staircase limit in surface quasigeostrophic turbulence

Surface buoyancy gradients over a quasigeostrophic fluid permit the existence of surface-trapped Rossby waves. The interplay of these Rossby waves with surface quasigeostrophic turbulence results in latitudinally inhomogeneous mixing that, under certain conditions, culminates in a surface buoyancy staircase: a meridional buoyancy profile consisting of mixed-zones punctuated by sharp buoyancy gradients, with eastward jets centred at the sharp gradients and weaker westward flows in between. In this article, we investigate the emergence of this buoyancy staircase limit in surface quasigeostrophic turbulence and we examine the dependence of the resulting dynamics on the vertical stratification. Over decreasing stratification [$\mathrm{d}N(z)/\mathrm{d}z\leq0$, where $N(z)$ is the buoyancy frequency], we obtain flows with a longer interaction range (than in uniform stratification) and highly dispersive Rossby waves. In the staircase limit, we find straight jets that are perturbed by eastward propagating along jet waves, similar to two-dimensional barotropic $\beta$-plane turbulence. In contrast, over increasing stratification [$\mathrm{d}N(z)/\mathrm{d}z\geq0$], we obtain flows with shorter interaction range and weakly dispersive Rossby waves. In the staircase limit, we find sinuous jets with large latitudinal meanders whose shape evolves in time due to the westward propagation of weakly dispersive along jet waves. These along jet waves have larger amplitudes over increasing stratification than over decreasing stratification, and, as a result, the ratio of domain-averaged zonal to meridional speeds is two to three times smaller over increasing stratification than over decreasing stratification. Finally, we find that, for a given Rhines wavenumber, jets over increasing stratification are closer together than jets over decreasing stratification.

==> Jet formation in SQG/PersonalDef.tex <==



% Personal Defintions
\newcommand{\abs}[1]{\left \lvert #1 \right\rvert} % for absolute value
\newcommand{\norm}[1]{\lVert #1 \rVert} % for absolute value
\newcommand{\avg}[1]{\left< #1 \right>} % for average
\newcommand{\inner}[2]{\left< #1, #2 \right>} % for average


\let\foo=\d % rename builtin command \d{} to \underdot{}
\renewcommand{\vec}[1]{\boldsymbol{#1}  } % for vectors
%\newcommand{\p}{\partial}
\newcommand{\lb}{\left}
\newcommand{\rb}{\right}
\renewcommand{\d}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}} % for derivatives
\newcommand{\dd}[2]{\frac{\mathrm{d}^2 #1}{\mathrm{d} #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} % for partial derivatives
\newcommand{\pdt}[2]{\frac{\partial^2 #1}{\partial #2^2}} % for double partial derivatives
\newcommand{\pdd}[3]{\frac{\partial^2 #1}{\partial #2 \partial#3}} % for double partial derivatives
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}
	\right)_{#3}} % for thermodynamic partial derivatives
\newcommand{\fd}[2]{\frac{\delta #1}{\delta #2}} % for functional derivatives
\newcommand{\fdd}[2]{\frac{\delta^2 #1}{\delta #2^2}} % for second partial derivatives
\newcommand{\grad}[1]{\vec{\nabla} #1} % for gradient
\let\divsymb=\div % rename builtin command \div to \divsymb
\renewcommand{\div}[1]{ \vec{\nabla} \cdot #1} % for divergence
\newcommand{\divh}[1]{ \vec{\nabla}_z \cdot #1} % for divergence
\newcommand{\lap}{\nabla^2} % for laplacian 
\newcommand{\laptwo}{\nabla^4} % for laplacian squared 
\newcommand{\lapz}{\nabla_z^2} % for laplacian 
\newcommand{\curl}[1]{\vec{\nabla} \cross #1} % for curl
\newcommand{\curlh}[1]{\vec{\nabla}_z \cross #1} % for curl
\newcommand{\D}[2]{\frac{D #1}{D #2}} % for Lagrangian derivatives
\newcommand{\cross}{\wedge}  % \cross for cross product
\renewcommand{\bar}{\overline} % \bar for writing an overline
\newcommand{\unit}[1]{\hat{\vec{#1}}}
\newcommand{\dV}{d^3 \vec x \ }
\newcommand{\dVt}{d^2 \vec x \ }
\newcommand{\dVn}[1]{d^#1 \vec x \ }
\newcommand{\dVa}{ d^3\vec a \ }
\newcommand{\J}[2]{ J\left(#1,#2\right) }

\newcommand{\reff}[1]{ \left(\ref{#1}\right)} % for divergence

%\newcommand{\ov}[1]{\overline{#1} }
\newcommand{\ov}[1]{{#1}^\ast }

\newcommand{\wh}[1]{\widehat{#1} }

